Magnetic Phases of Spatially-Modulated Spin-1 Chains in Rydberg Excitons: Classical and Quantum Simulations

In this work, we study the magnetic phases of a spatially-modulated chain of spin-1 Rydberg excitons. Using the Density Matrix Renormalization Group (DMRG) technique we study various magnetic and topologically nontrivial phases using both single-particle properties like local magnetization and quantum entropy as well as many-body ones like pair-wise N\'eel and long-range string correlations. In particular, we investigate the emergence and robustness of Haldane phase, a topological phase of anti-ferromagnetic spin-1 chains. Further, we devise a hybrid quantum algorithm employing Restricted Boltzmann Machine to simulate the ground state of such a system which shows very good agreement with the results of exact diagonalization (ED) and DMRG.

==> colors.tex <==
\definecolor{blue}{rgb}{0.38, 0.51, 0.71} %glaucous, 97,130,181, #6182B5
\definecolor{darkblue}{RGB}{17, 42, 60} % 112A3C
\definecolor{red}{RGB}{175, 49, 39} % AF3127

\definecolor{orange}{RGB}{217, 156, 55} % D99C37
\definecolor{green}{RGB}{144, 169, 84} % 90A954
\definecolor{palegreen}{RGB}{197, 184, 104} % C5B868

\definecolor{yellow}{RGB}{250, 199, 100} % FAC764
\definecolor{brokenwhite}{RGB}{218, 192, 166} % DAC0A6
\definecolor{brokengrey}{rgb}{0.77, 0.76, 0.82} % {196,194,209}, C4C2D1


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
